An Integrated Design Pipeline for Tactile Sensing Robotic Manipulators

Traditional robotic manipulator design methods require extensive, time-consuming, and manual trial and error to produce a viable design. During this process, engineers often spend their time redesigning or reshaping components as they discover better topologies for the robotic manipulator. Tactile sensors, while useful, often complicate the design due to their bulky form factor. We propose an integrated design pipeline to streamline the design and manufacturing of robotic manipulators with knitted, glove-like tactile sensors. The proposed pipeline allows a designer to assemble a collection of modular, open-source components by applying predefined graph grammar rules. The end result is an intuitive design paradigm that allows the creation of new virtual designs of manipulators in a matter of minutes. Our framework allows the designer to fine-tune the manipulator's shape through cage-based geometry deformation. Finally, the designer can select surfaces for adding tactile sensing. Once the manipulator design is finished, the program will automatically generate 3D printing and knitting files for manufacturing. We demonstrate the utility of this pipeline by creating four custom manipulators tested on real-world tasks: screwing in a wing screw, sorting water bottles, picking up an egg, and cutting paper with scissors.

==> text/old_intro.tex <==
\pulkit{Main Issues: 
\begin{itemize}
    \item We are assuming access to pre-tested components. Why does grammar help combining these components into designs faster / intuititvely is not explained. It is simply asserted, but not quantified. We must explain the intuition behind grammar. 
    \item Its importat to explicitly point out what pre-tested means, what constraints a new part in the grammar needs to satisfy and the choice of context-free/context-sensitive grammar.
    \item Is our contribution just the grammar or does it also relate with specific way of constructing components? 
\end{itemize}}

% Contributions: (1) integrated design system for designing manipulators with different topologies for different applications, (2) integrated manufacturing method for making manipulators with integrated sensing, (3) demonstration with important applications}
At present, designing robotic manipulators with integrated tactile sensing is both time-consuming and manual. Following the traditional design method, one typically brainstorms designs to solve a specific task (or set of tasks), prototypes a selection of brainstormed designs, chooses the most promising prototype(s), and repetitively iterates prototyping until a final, successful design is achieved. From start to finish, depending on complexity, it may take months or years to produce a high quality product. Additionally, during and after the design phase, altering the topology of a manipulator is generally time-intensive as re-shaped pieces may no longer perform mechanically: all interfacing components must be manually re-modeled and tested to fit the new form factor, tactile sensors must be re-incorporated in the new design, and a new set of manufacturing instructions must be manually generated.

% Much research is currently devoted to developing robotic hands, whether for home or industrial use. While home robots often require hands to perform a more versatile array of tasks, companies have expressed preference for highly specialized manipulators to optimize their supply chains and decrease production and packaging time. The need for the systematic design of numerous manipulators is ill-suited to the typical month- or year-long development cycle for current manipulators \lara{cite}. The traditional trial-and-error iterative design method is centered around a certain task or set of tasks. Hence, creating a new manipulator for a different purpose requires restarting from scratch and repeating the entire design process. \mike{I think the comparison of industrial vs home use manipulators is a bit confusing and does not properly motivate the work. Currently, designing robotic manipulators with integrated tactile sensing is a time consuming and manual process. Typically, altering the topology of the manipulator requires significant redesign. Typically, to change the topology, the process involves redesigning the mechanical assembly, reintegrating the tactile sensors, and producing a new set of manufacturing instructions. I would point to examples that show how manual the process is and how currently design and manufacturing take place.}

We propose a robust, interactive design and manufacturing pipeline to streamline the design process and present a platform for designing manipulators in a matter of hours or days. We propose an integrated design system for designing manipulators with pressure sensing and different topologies for specialized applications. \pulkit{Motivation for the approach is lacking. We say current methods are not as effective, our method is faster, but we don't say why our method is faster. Its necessary to explain before describing the method.}
\lara{Hmm that makes sense but since a lot of the advantages derive from the grammar and the grammar hasn't been explained, how could I introduce the motivation? I discuss it (well, advantages, not necessarily motivation) a couple paragraphs later and could move it up. However, I'm concerned that it references the method too much.}
Given our pre-tested \pulkit{tested for what?}, open-source ``lego kit" of sub-component 3D models and given grammar rules for assembling those components in different configurations, users can apply the assembly rules to instantly create many different graphs (configurations and styles) of working robotic manipulators. After creating the desired configuration, they may topologically deform (i.e., lengthen, widen, and otherwise distort) their manipulator models according to the desired finger and hand size for their tasks. To add integrated sensing, users can selectively place tactile sensing points on their 3D hand model. The program is integrated with manufacturing methods: once the manipulator is virtually completed, the pipeline will automatically \mike{Is it automatic at this point?} convert the hand model to manufacturing files with instructions. An illustration of this workflow can be seen in Figure \ref{fig:workflow}.

We applied the above described method to creating 3D printed, cable-driven robotic hands to grasp a variety of objects. Where necessary, they are covered with knitted tactile sensors, worn almost like gloves.
% These sensors are manufactured on a digital knitting machine, with coaxial piezoresistive fibers manually interwoven. The special fibers overlap to create sensing points based on techniques from previous work~\cite{luo2021learning}.
Because of their conformal nature, these sensors can be easily added over the grippers and adapted to any manipulator shape. In contrast, traditional sensors, such as GelSight~\cite{yuan2017gelsight} or bubble grippers~\cite{BubbleGripper}, require the manipulator to be designed around the sensors, leading to bulky or sub-optimal design geometry.

The structure of the pipeline provides numerous benefits over the traditional design method. (1) The inputted sub-components are pre-tested, guaranteeing that initial designs will perform. \pulkit{Seems like a repetition?} This reduces trial and error in the design process and allows the designer to focus on improving form rather than functionality. (2) The grammar rules simplify re-design by allowing new and completely different manipulators to be constructed in a matter of seconds where each of the designs produced are immediately functional \pulkit{Its unclear why grammar helps to speed up the design process}. These manipulators can then be topologically deformed as desired \pulkit{mention through the API, that it can be done intuitively}. (3) Due to the conformal and geometrically scalable nature of the knitted sensors, all manipulators produced by the program can have integrated sensing, which can be specified by a few clicks of the cursor. The user does not have to design around sensor geometry, and the sensor manufacturing instructions are automatically generated by the program. \pulkit{This needs to move up} (4) The computer-based grammar and graph method as well as the computer-automated tactile sensing in our design pipeline allow easy integration with ML, AI, computational simulation, and other software for computational exploration of the design space, geometry optimization, and control simulation and optimization. \mike{I would suggest making this paragraph more about how the graph and grammar help automate the design process, this is the key contribution in this work. You can mention that it makes design optimization easier, but I would limit it to not more than a sentence.} \lara{old paragraph deleted and replaced with advantages of our system}

Four tasks with practical application were selected to demonstrate the breadth of design possibilities and efficacy of this system. Using the method described above, four separate manipulators are designed to (1) screw on and off a wing nut, (2) pour water from a bottle at a desired rate, (3) pick up an egg, and (4) cut paper with scissors.
